Guidelines for the Computational Testing of Machine Learning approaches to Vehicle Routing Problems

Despite the extensive research efforts and the remarkable results obtained on Vehicle Routing Problems (VRP) by using algorithms proposed by the Machine Learning community that are partially or entirely based on data-driven analysis, most of these approaches are still seldom employed by the Operations Research (OR) community. Among the possible causes, we believe, the different approach to the computational evaluation of the proposed methods may play a major role. With the current work, we want to highlight a number of challenges (and possible ways to handle them) arising during the computational studies of heuristic approaches to VRPs that, if appropriately addressed, may produce a computational study having the characteristics of those presented in OR papers, thus hopefully promoting the collaboration between the two communities.

==> teximgs/boxplot.tex <==
	\scriptsize
	\makeatletter
	\pgfplotsset{
		boxplot/draw/average/.code={ % the bulk part of this is the default, found in the manual
			\draw [/pgfplots/boxplot/every average/.try]
			\pgfextra
			% do NOT use \draw[mark=*] plot coordinates because
			% boxplots uses the same plot handler to draw its
			% outliers.
			\pgftransformshift{%
				% basic level access to ’boxplot box cs’:
				\pgfplotsboxplotpointabbox
				{\pgfplotsboxplotvalue{average}}
				{0.5}%
			}%
			%\pgfuseplotmark{\tikz@plot@mark}%
			\endpgfextra
			;
			% the following line is the only new addition
			%\node[right,font=\tiny] at (boxplot box cs: \boxplotvalue{average}, 0.95) {\pgfmathprintnumber{\boxplotvalue{average}}};
		}
	}
	\makeatother
	\begin{tikzpicture}
	\begin{axis}
	[
	clip=false,
	boxplot/draw direction=y,
	boxplot/variable width,
	boxplot/every median/.style={black,very thick,solid},
	xmin=0.5,xmax=2.5,
	width=1.00\textwidth,
	height=0.33\textheight,
	ylabel style={align=center}, 
	y tick label style={align=right},
	x tick label style={align=center},
	xtick={1, 1.5, 2},
	ymajorgrids=true,
	grid style=dashed,
	xticklabels={{\small HGS-CVRP}, {\small SISR}, {\small OR-Tools}}, xticklabel style={rotate=0}, ylabel={\footnotesize Average \% gap},
	scatter/classes={ a={mark=star}, b={mark=*}}]

	% HGS
	\addplot[
	mark=*, mark size=0.5pt,boxplot,
	boxplot prepared={draw position=1, 
	lower whisker=0.00, 
	lower quartile=0.00,  
	median= 0.05, 
	upper quartile=0.185, 
	upper whisker=0.440,sample size=1}
	] coordinates{ (1, 0.55) (1, 0.49) (1, 0.54) };


	% SISR
	\addplot[
	mark=*, mark size=0.5pt,boxplot,
	boxplot prepared={draw position=1.5, 
	lower whisker=0.00, 
	lower quartile=0.07, 
	median=0.17, 
	upper quartile=0.27, 
	upper whisker=0.45,
	sample size=1}
	] coordinates{ (1.5, 1.63) (1.5, 0.58) };
	
	
	%OR-Tools
	\addplot[
	mark=*, mark size=0.5pt,boxplot,
	boxplot prepared={
	draw position=2,
	lower whisker=0.38,
	lower quartile=2.835,
	median=3.945,
	upper quartile=4.965,
	upper whisker=8.040,
	sample size=1}
	] coordinates{(2, 8.62)};
	
		
	

	\end{axis}
	\end{tikzpicture}
